Proximal Ranking Policy Optimization for Practical Safety in Counterfactual Learning to Rank

Counterfactual learning to rank (CLTR) can be risky and, in various circumstances, can produce sub-optimal models that hurt performance when deployed. Safe CLTR was introduced to mitigate these risks when using inverse propensity scoring to correct for position bias. However, the existing safety measure for CLTR is not applicable to state-of-the-art CLTR methods, cannot handle trust bias, and relies on specific assumptions about user behavior. We propose a novel approach, proximal ranking policy optimization (PRPO), that provides safety in deployment without assumptions about user behavior. PRPO removes incentives for learning ranking behavior that is too dissimilar to a safe ranking model. Thereby, PRPO imposes a limit on how much learned models can degrade performance metrics, without relying on any specific user assumptions. Our experiments show that PRPO provides higher performance than the existing safe inverse propensity scoring approach. PRPO always maintains safety, even in maximally adversarial situations. By avoiding assumptions, PRPO is the first method with unconditional safety in deployment that translates to robust safety for real-world applications.

==> copyright.tex <==
% !TEX root = ./2024-crm-ppo.tex

\copyrightyear{2024}
\acmYear{2024}
\setcopyright{rightsretained}
\acmConference[CIKM '24]{Proceedings of the 33rd ACM International Conference on Information and Knowledge Management}{October 21--25, 2024}{Boise, ID, USA}
\acmBooktitle{Proceedings of the 33rd ACM International Conference on Information and Knowledge Management (CIKM '24), October 21--25, 2024, Boise, ID, USA}
\acmDOI{10.1145/3627673.3679531}
\acmISBN{979-8-4007-0436-9/24/10}

\usepackage{etoolbox}
\makeatletter
\patchcmd{\maketitle}{\@copyrightpermission}{
  \begin{minipage}{0.3\columnwidth}
    \href{http://creativecommons.org/licenses/by/4.0/}{\includegraphics[width=0.90\textwidth]{./figures/4ACM-CC-by-88x31.eps}}
  \end{minipage}\hfill
  \begin{minipage}{0.7\columnwidth}
    \href{http://creativecommons.org/licenses/by/4.0/}{This work is licensed under a Creative Commons Attribution International 4.0 License.}
  \end{minipage}
  \vspace{5pt}
}{}{}
\makeatother


==> sections/01-introduction.tex <==
% !TEX root = ../2024-crm-ppo.tex

\section{Introduction}\label{sect:intro}

\Ac{CLTR}~\cite{joachims2017unbiased, wang2016learning, oosterhuis2020learning,gupta2024unbiased} concerns the optimization of ranking systems based on user interaction data using \ac{LTR} methods~\cite{liu2009learning}.
A main advantage of \ac{CLTR} is that it does not require manual relevance labels, which are costly to produce~\citep{qin2010letor,chapelle2011yahoo} and often do not align with actual user preferences~\cite{sanderson2010test}.
Nevertheless, \ac{CLTR} also brings significant challenges since user interactions only provide a heavily biased form of implicit feedback~\citep{gupta2024unbiased}.
User clicks are affected by many different factors, for example, the position at which an item is displayed  in a ranking~\citep{wang2018position, craswell2008experimental}.
Thus, click frequencies provide a biased indication of relevance, that is often more representative of how an item was displayed than actual user preferences~\citep{agarwal2019addressing, wang2016learning}.

To correct for this bias, early \ac{CLTR} applied \ac{IPS}, which weights clicks inversely to the estimated effect of position bias~\cite{joachims2017unbiased, wang2016learning}.
Later work expanded this approach to correct for other forms of bias, e.g., item-selection bias~\citep{oosterhuis2020policy, ovaisi2020correcting} and trust bias~\citep{agarwal2019addressing, vardasbi2020inverse}, and more advanced \ac{DR} estimation~\citep{oosterhuis2022doubly}.
Using these methods, standard \ac{CLTR} aims to create an unbiased estimate of relevance (or user preference) from click frequencies.
In other words, their goal is to output an estimate per document with an expected value that is equal to their relevance.

However, unbiased estimates of \ac{CLTR} have their limitations.
Firstly, they assume a model of user behavior and require an accurate estimate of this model.
If the assumed model is incorrect~\citep{vardasbi2020inverse, oosterhuis2020policy} or its estimated parameters are inaccurate~\citep{joachims2017unbiased, oosterhuis2022doubly}, then their unbiasedness is not guaranteed.
Secondly, even when unbiased, the estimates are subject to variance~\cite{oosterhuis2022reaching}.
As a result, the actual estimated values are often erroneous, especially when the available data is sparse~\citep{oosterhuis2022doubly, gupta2023safe}.
Accordingly, unbiased \ac{CLTR} does not guarantee that the ranking models it produces have optimal performance~\cite{oosterhuis2022reaching}.

\header{Safe \acl{CLTR}}
There are risks involved in applying \ac{CLTR} in practice. 
In particular, there is a substantial risk that a learned ranking model is deployed that degrades performance compared to the previous production system~\citep{gupta2023safe,oosterhuis2021robust,jagerman2020safe}.
This can have negative consequences to important business metrics, making \ac{CLTR} less attractive to practitioners.
To remedy this issue, a \emph{safe} \ac{CLTR} approach was proposed by \citet{gupta2023safe}.
Their approach builds on IPS-based \ac{CLTR} and adds exposure-based risk regularization, which keeps the learned model from deviating too much from a given safe model.
Thereby, under the assumption of a position-biased user model, the safe \ac{CLTR} approach can guarantee an upper bound on the probability of the model being worse than the safe model.

\header{Limitations of the current safe \ac{CLTR} method}
Whilst safe \ac{CLTR} is an important contribution to the field, it has two severe limitations -- both are addressed by this work.
Firstly, the existing approach is only applicable to \ac{IPS} estimation, which is no longer the state-of-the-art in the field~\citep{gupta2024unbiased}, and it assumes a rank-based position bias model~\citep{craswell2008experimental, wang2016learning}, the most basic user behavior model in the field.
Secondly, because its guarantees rely on assumptions about user behavior, it can only provide a conditional notion of safety.
Moreover, since user behavior can be extremely heterogeneous, it is unclear whether a practitioner could even determine whether the safety guarantees would apply to their application.

% \header{Safe \acl{DR} \ac{CLTR}}
\header{Main contributions}
Our first contribution addresses the mismatch between the existing safe \ac{CLTR} approach and recent advances in \ac{CLTR}.
We propose a novel generalization of the exposure-based regularization term that provides safety guarantees for both \ac{IPS} and \ac{DR} estimation, also under more complex models of user behavior that cover both position and trust bias.
Our experimental results show that our novel method reaches higher levels of performance significantly faster, while avoiding any notable decreases of performance.
This is especially beneficial since \ac{DR} is known to have detrimental performance when very little data is available~\citep{oosterhuis2022doubly}.

Our second contribution provides an unconditional notion of safety. We take inspiration from advances in \ac{RL}~\cite{wang2020truly,schulman2017proximal,liu2019neural,wang2019trust,queeney2021generalized} and propose the novel \acfi{PRPO} method.
\ac{PRPO} removes incentives for \ac{LTR} methods to rank documents too much higher than a given safe ranking model would.
Thereby, \ac{PRPO} imposes a limit on the performance difference between a learned model and a safe model, in terms of standard ranking metrics.
Importantly, \ac{PRPO} is easily applicable to \emph{any} gradient-descent-based \ac{LTR} method, and makes \emph{no assumptions} about user behavior.
In our experiments, \ac{PRPO} prevents any notable decrease in performance even under extremely adversarial circumstances, where other methods fail.
Therefore, we believe \ac{PRPO} is the first \emph{unconditionally} safe \ac{LTR} method. % in the field.

Together, our contributions bring important advances to the theory of safe \ac{CLTR}, by proposing a significant generalization of the existing approach with theoretical guarantees, and the practical appeal of \ac{CLTR}, with the first robustly safe \ac{LTR} method: \ac{PRPO}.
All source code to reproduce our experimental results is available at: 
\url{https://github.com/shashankg7/cikm-safeultr}.
%\href{https://anonymous.4open.science/r/cikm-safeultr-3E6C}{cikm24 safe cltr}.

\vspace{-1.1mm}


==> sections/02-related-works.tex <==
% !TEX root = ../2024-crm-ppo.tex

\section{Related Work}
\label{sec:relatedwork}
\textbf{\Acl{CLTR}.}
\citet{joachims2017unbiased} introduced the first method for \ac{CLTR}, a \ac{LTR} specific adaptation of \ac{IPS} from the bandit literature~\cite{swaminathan2015batch,joachims2016counterfactual,saito2021counterfactual,gupta2024optimal,gupta2023deep, gupta2024first} to correct for position bias.
They weight each user interaction according to the inverse of its examination probability, i.e., its inverse propensity, during learning to correct for the position bias in the logged data. 
This weighting will remove the effect of position bias from the final ranking policy.
\citet{oosterhuis2020policy} extended this method for the top-$K$ ranking setting with item-selection bias, where any item placed outside the top-$K$ positions gets zero exposure probability, i.e., an extreme form of position bias. 
They proposed a policy-aware propensity estimator, where the propensity weights used in \ac{IPS} are conditioned on the logging policy used to collect the data. 

\citet{agarwal2019addressing} introduced an extension of \ac{IPS}, known as Bayes-IPS, to correct for \textit{trust bias}, an extension of position-bias, with false-positive clicks at the higher ranks, because of the users' trust in the search engine. 
\citet{vardasbi2020inverse} proved that Bayes-IPS cannot correct for trust bias and introduced an affine-correction method and unbiased estimator. 
\citet{oosterhuis2021unifying} combined the affine-correction with a policy-aware propensity estimator to correct for trust bias and item-selection bias simultaneously.
Recently, \citet{oosterhuis2022doubly} introduced a \ac{DR}-estimator for \ac{CLTR}, which combines the existing \ac{IPS}-estimator with a regression model to overcome some of the challenges with the \ac{IPS}-estimator. 
The proposed \ac{DR}-estimator corrects for item-selection and trust biases, with lower variance and improved sample complexity. 

\header{Safe policy learning from user interactions}
In the context of offline evaluation for contextual bandits, \citet{thomas2015high} introduced a high-confidence off-policy evaluation framework.
A confidence interval is defined around the empirical off-policy estimates, and there is a high probability that the \textit{true} utility can be found in the interval. 
\citet{jagerman2020safe} extended this framework for safe deployment in the contextual bandit learning setup. 
The authors introduce a \ac{SEA} method that selects with high confidence between a safe behavior policy and the newly learned policy. 
In the context of \ac{LTR}, \citet{oosterhuis2021robust} introduced the \ac{GENSPEC} method, which safely selects between a feature-based and tabular \ac{LTR} model. 
For off-policy learning, \citet{swaminathan2015batch} introduced a \ac{CRM} framework for the contextual bandit setup. 
They modify the \ac{IPS} objective for bandits to include a regularization term, which explicitly controls for the variance of the \ac{IPS}-estimator during learning, thereby overcoming some of the problems with the high-variance of \ac{IPS}.
\citet{wu2018variance} extended the \ac{CRM} framework by using a \textit{risk} regularization, which penalizes mismatches in the action probabilities under the new policy and the behavior policy. 
\citet{gupta2023safe} made this general safe deployment framework effective in the \ac{LTR} setting. 
They proposed an exposure-based risk regularization method where the difference in the document exposure distribution under the new and logging policies is penalized. 
When click data is limited, risk regularization ensures that the performance of the new policy is similar to the logging policy, ensuring safety. 

To the best of our knowledge, the method proposed by~\citet{gupta2023safe} is the only method for safe policy learning in the \ac{LTR} setting. 
While it guarantees safe ranking policy optimization, it has two main limitations:
\begin{enumerate*}[label=(\roman*)]
        \item It is only applicable to the \ac{IPS} estimator; and  
        \item under the position-based click model assumption, the most basic click model in the \ac{CLTR} literature~\citep{joachims2017unbiased, oosterhuis2020learning, gupta2024unbiased}. 
\end{enumerate*} 

\header{Proximal policy optimization} 
In the broader context of \ac{RL}, \acfi{PPO} was introduced as a policy gradient method for training \ac{RL} agents to maximize long-term rewards~\cite{wang2020truly,schulman2017proximal,liu2019neural,wang2019trust,queeney2021generalized}.
\Ac{PPO} clips the importance sampling ratio of action probability under the new policy and the current behavior policy, and thereby, it prevents the new policy to deviate from the behavior policy by more than a certain margin.
\ac{PPO} is not directly applicable to \ac{LTR}, for the same reasons that the \ac{CRM} framework is not: the combinatorial action space of \ac{LTR} leads to extremely small propensities that \ac{PPO} cannot effectively manage~\cite{gupta2023safe}.
%In the context of \ac{LTR}, \ac{PPO} is not directly applicable since the actions in the ranking context are combinatorial, resulting in extremely small action propensities ($\pi(A \mid X)$), resulting in a high-variance and unstable estimator~\cite{gupta2023safe}.


==> sections/table.tex <==
\begin{tabular}{ l ccc  ccc ccc}
 \toprule
&\multicolumn{3}{c}{ Yahoo! Webscope}
&\multicolumn{3}{c}{ MSLR-WEB30k}
&\multicolumn{3}{c}{ Istella}\\
\cmidrule(r){2-4}
\cmidrule(r){5-7}
\cmidrule{8-10}
& $N=4\cdot10^2$&  $N=4 \cdot 10^7$ &  $N=10^9$&  $N=4 \cdot 10^2$ &  $N=4 \cdot 10^7$ &  $N=10^9$&  $N=4 \cdot 10^2$ &  $N=4 \cdot 10^7$ &  $N=10^9$\\
 \midrule
% &\multicolumn{9}{c}{  \emph{Top-5 Setting with Known Bias Parameters} } \\ \midrule
\multicolumn{1}{l}{ Logging} &  0.677 \phantom{\small(0.000)}\phantom{$^{\tiny -}$}  &  0.677 \phantom{\small(0.000)}\phantom{$^{\tiny -}$}  &  0.677 \phantom{\small(0.000)}\phantom{$^{\tiny -}$}  &  0.435 \phantom{\small(0.000)}\phantom{$^{\tiny -}$}  &  0.435 \phantom{\small(0.000)}\phantom{$^{\tiny -}$}  &  0.435 \phantom{\small(0.000)}\phantom{$^{\tiny -}$}  &  0.635 \phantom{\small(0.000)}\phantom{$^{\tiny -}$}  &  0.635 \phantom{\small(0.000)}\phantom{$^{\tiny -}$}  &  0.635 \phantom{\small(0.000)}\phantom{$^{\tiny -}$}  \\ 
\multicolumn{1}{l}{ Skyline}&  0.727 \phantom{\small(0.000)}\phantom{$^{\tiny -}$} &  0.727 \phantom{\small(0.000)}\phantom{$^{\tiny -}$} &  0.727 \phantom{\small(0.000)}\phantom{$^{\tiny -}$} &  0.479 \phantom{\small(0.000)}\phantom{$^{\tiny -}$} &  0.479 \phantom{\small(0.000)}\phantom{$^{\tiny -}$} &  0.479 \phantom{\small(0.000)}\phantom{$^{\tiny -}$} &  0.714 \phantom{\small(0.000)}\phantom{$^{\tiny -}$} &  0.714 \phantom{\small(0.000)}\phantom{$^{\tiny -}$} &  0.714 \phantom{\small(0.000)}\phantom{$^{\tiny -}$} \\ \midrule
\multicolumn{1}{l}{ Naive}&  0.652 \small (0.021)$^{\tiny \blacktriangledown}$ &  0.694 \small (0.000)$^{\tiny \blacktriangledown}$ &  0.695 \small (0.000)$^{\tiny \blacktriangledown}$ &  0.353 \small (0.003)$^{\tiny \blacktriangledown}$ &  0.448 \small (0.000)$^{\tiny \blacktriangledown}$ &  0.448 \small (0.001)$^{\tiny \blacktriangledown}$ &  0.583 \small (0.007)$^{\tiny \blacktriangledown}$ &  0.661 \small (0.001)$^{\tiny \blacktriangledown}$ &  0.661 \small (0.001)$^{\tiny \blacktriangledown}$  \\ 
 \multicolumn{1}{l}{Action IPS}&  0.656 \small (0.008)$^{\tiny \blacktriangledown}$ &  0.701 \small (0.001)$^{\tiny \blacktriangledown}$ &  0.701 \small (0.001)$^{\tiny \blacktriangledown}$ &  0.359 \small (0.007)$^{\tiny \blacktriangledown}$ &  0.448 \small (0.001)$^{\tiny \blacktriangledown}$ &  0.448 \small (0.001)$^{\tiny \blacktriangledown}$ &  0.578 \small (0.004)$^{\tiny \blacktriangledown}$ &  0.671 \small (0.001)$^{\tiny \blacktriangledown}$ &  0.671 \small (0.002)$^{\tiny \blacktriangledown}$  \\ 
 \multicolumn{1}{l}{Action \ac{CRM}}&  0.617 \small (0.004)$^{\tiny \blacktriangledown}$ &  0.698 \small (0.001)$^{\tiny \blacktriangledown}$ &  0.700 \small (0.001)$^{\tiny \blacktriangledown}$ &  0.359 \small (0.005)$^{\tiny \blacktriangledown}$ &  0.448 \small (0.001)$^{\tiny \blacktriangledown}$ &  0.449 \small (0.001)$^{\tiny \blacktriangledown}$ &  0.449 \small (0.013)$^{\tiny \blacktriangledown}$ &  0.668 \small (0.002)$^{\tiny \blacktriangledown}$ &  0.672 \small (0.001)$^{\tiny \blacktriangledown}$  \\ 
 \multicolumn{1}{l}{Exp. IPS}&  0.659 \small (0.010)$^{\tiny \blacktriangledown}$ &  \textbf{0.723 \small (0.001)}$^{\tiny \star}$ &  \textbf{0.730 \small (0.001)}$^{\tiny \star}$ &  0.389 \small (0.014)$^{\tiny \blacktriangledown}$ &  \textbf{0.474 \small (0.001)}$^{\tiny \star}$ &  \textbf{0.481 \small (0.001)}$^{\tiny \star}$ &  0.576 \small (0.010)$^{\tiny \blacktriangledown}$ &  \textbf{0.696 \small (0.001)}$^{\tiny \star}$ &  \textbf{0.706 \small (0.001)}$^{\tiny \star}$  \\  
 \multicolumn{1}{l}{Exp. \ac{CRM}}&  \textbf{0.677 \small (0.001)}\phantom{$^{\tiny -}$} &  \textbf{0.723 \small (0.001)}\phantom{$^{\tiny -}$} &  \textbf{0.730 \small (0.000)}\phantom{$^{\tiny -}$} &  \textbf{0.434 \small (0.001)}\phantom{$^{\tiny -}$} &  \textbf{0.473 \small (0.001)}\phantom{$^{\tiny -}$} &  \textbf{0.480 \small (0.001)}\phantom{$^{\tiny -}$} &  \textbf{0.635 \small (0.001)}\phantom{$^{\tiny -}$} &  \textbf{0.695 \small (0.001)}\phantom{$^{\tiny -}$} &  \textbf{0.706 \small (0.001)}\phantom{$^{\tiny -}$}  \\ 
 \bottomrule
\end{tabular}
